On the noncommutative residue for pseudodifferential operators with log-polyhomogeneous symbols

We study various aspects of the noncommutative residue for an algebra of pseudodifferential operators whose symbols have an expansion $a\sim \sum_{j=0}^\infty a_{m-j}, a_{m-j}(x,\xi)=\sum_{l=0}^k a_{m-j,l}(x,\xi) \log^l|\xi|,$ where $a_{m-j,l}$ is homogeneous in $\xi$ of degree $m-j$. We will explain why this algebra of pseudodifferential operators is natural. For a pseudodifferential operator in this class, $A$, and a classical elliptic pseudodifferential operator, $P$, we show that the generalized zeta-function $\Tr(AP^{-s})$ has a meromorphic continuation to the whole complex plane, however possibly with higher order poles. Our algebra of operators has a bigrading given by the order and the highest log-power occuring in the symbol expansion. We construct "higher" noncommutative residue functionals on the subspaces given by the log-grading. However, in contrast to the classical case we prove that the whole algebra does not admit any nontrivial traces. Finally we show that the analogue of the Kontsevich-Vishik trace also exists on our algebra. Our method also provides an alternative approach to the Kontsevich-Vishik trace.

==> abstract.tex <==

\begin{footnotesize}{\bf Abstract. }
We study various aspects of the noncommutative residue for
an algebra of pseudodifferential operators whose symbols have
an expansion
$$a\sim \sum_{j=0}^\infty a_{m-j},\quad 
   a_{m-j}(x,\xi)=\sum_{l=0}^k a_{m-j,l}(x,\xi)\log^l|\xi|,$$
where $a_{m-j,l}$ is homogeneous in $\xi$ of degree $m-j$.
We call these symbols \poly. We will explain why this
algebra of pseudodifferential operators is natural.

We study \poly\ functions on symplectic cones and 
generalize the symplectic residue of {\sc Guillemin} to these functions.
Similarly as for homogeneous functions, for a \poly\ function 
this symplectic residue is an obstruction against being a
sum of Poisson brackets. 

For a pseudodifferential operator with \poly\
symbol, $A$, and a classical elliptic pseudodifferential operator,
$P$, we show that the generalized $\zeta$--function 
$\Tr(AP^{-s})$ has a meromorphic
continuation to the whole complex plane, however possibly with
higher order poles.

Our algebra of operators has a bigrading given by the order
and the highest log--power occuring in the symbol expansion.
We construct "higher" noncommutative residue functionals on the
subspaces given by the log--grading. However, in contrast
to the classical case we prove that the whole algebra does not admit 
any nontrivial traces.

Finally we show that the analogue of the {\sc Kontsevich--Vishik} trace
also exists on our algebra. Our method also provides an alternative
approach to the {\sc Kontsevich--Vishik} trace.

\bigskip
{\bf 1991 Mathematics Subject Classification.} \subjclass
%\footnotetext{{\it Keywords and phrases.} \keywords}  
\end{footnotesize}


